Malware Makeover: Breaking ML-based Static Analysis by Modifying Executable Bytes

Motivated by the transformative impact of deep neural networks (DNNs) in various domains, researchers and anti-virus vendors have proposed DNNs for malware detection from raw bytes that do not require manual feature engineering. In this work, we propose an attack that interweaves binary-diversification techniques and optimization frameworks to mislead such DNNs while preserving the functionality of binaries. Unlike prior attacks, ours manipulates instructions that are a functional part of the binary, which makes it particularly challenging to defend against. We evaluated our attack against three DNNs in white- and black-box settings, and found that it often achieved success rates near 100%. Moreover, we found that our attack can fool some commercial anti-viruses, in certain cases with a success rate of 85%. We explored several defenses, both new and old, and identified some that can foil over 80% of our evasion attempts. However, these defenses may still be susceptible to evasion by attacks, and so we advocate for augmenting malware-detection systems with methods that do not rely on machine learning.

==> figures/whitebox-attacks-kaggle.tex <==
\begin{figure*}[!ht]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figures/whitebox-attacks-malware-binaries.pdf}
    \caption{Malicious binaries}
  \end{subfigure}

  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figures/whitebox-attacks-benign-binaries.pdf}
    \caption{Benign binaries}
  \end{subfigure}

  \caption{\label{fig:wbattackskaggle}Attack success rates in the white-box setting. For
    each attack and \dnn{}, we show the percentage of misclassified malicious
    (a) and benign (b) binaries. The brigher section of each bar shows the percentage
    of binaries misclassified with high confidence. (Most binaries are misclassified with high confidence.)}
\end{figure*}


==> figures/whitebox-attacks-vtfeed-trends-models.tex <==
\begin{figure*}[!ht]
  \centering
  \begin{subfigure}{\textwidth}
    \makebox[\textwidth][c]{\includegraphics[width=1.0\textwidth]{figures/progress-model-trend-gef.pdf}}
    \caption{Binary Maliciousness - Budget}
  \end{subfigure}

  \begin{subfigure}{\textwidth}
    \makebox[\textwidth][c]{\includegraphics[width=1.0\textwidth]{figures/success-model-trend-gef.pdf}}
    \caption{Successful Misclassification - Budget}
  \end{subfigure}

  \caption{\label{fig:wbattacktrendsmodel}Attack Potency Comparison - A contrasting view showing the effectiveness over iteration for the whitebox attacks. Lines starting at top (resp., bottom) represent the progress of malicious (resp., benign) binaries over iterations.}
\end{figure*}


==> tables/test-samples.tex <==

\begin{table}
\small
  \begin{center}
  \begin{tabular}  {r | c c c}
    \toprule
    \vtfeed & \avastnet{} & \malconv{} & \ember{} \\ \midrule
    Benign & 100 & 100 & 100  \\
    Malicious & 100 & 100 & 100  \\
    \bottomrule
  \end{tabular}
  \caption{\label{tab:testsamples} The number of benign and malicious
    binaries used to test our attacks against the three \dnn{}s.}
\end{center}
\end{table}

